Crash-Stop Failures in Asynchronous Multiparty Session Types

Session types provide a typing discipline for message-passing systems. However, their theory often assumes an ideal world: one in which everything is reliable and without failures. Yet this is in stark contrast with distributed systems in the real world. To address this limitation, we introduce a new asynchronous multiparty session types (MPST) theory with crash-stop failures, where processes may crash arbitrarily and cease to interact after crashing. We augment asynchronous MPST and processes with crash handling branches, and integrate crash-stop failure semantics into types and processes. Our approach requires no user-level syntax extensions for global types, and features a formalisation of global semantics, which captures complex behaviours induced by crashed/crash handling processes. Our new theory covers the entire spectrum, ranging from the ideal world of total reliability to entirely unreliable scenarios where any process may crash, using optional reliability assumptions. Under these assumptions, we demonstrate the sound and complete correspondence between global and local type semantics, which guarantee deadlock-freedom, protocol conformance, and liveness of well-typed processes by construction, even in the presence of crashes.

==> evaluation.tex <==
\section{Evaluation}\label{sec:eval}

We evaluate our toolchain \theTool from two perspectives: \emph{expressivity}
and \emph{feasibility}. For expressivity, we use examples from the session type
literature, and extend them to include crash handling behaviour using two
patterns: failover and graceful failure. For feasibility, we show that our tool
generates \Scala code with negligible time, thanks to the guarantees from our
theory.

We note that we do \emph{not} evaluate the performance of the generated code.
The generated code uses the \Effpi concurrency library to
implement protocols,
and any performance indication would depend and reflect on the performance of
\Effpi,
instead of \theTool.

\subparagraph*{Expressivity}\label{sec:eval:expressivity}

\input{figs/resultsMetrics.tex}

We evaluate our methodology with examples in the session type literature:
\exampleName{PingPong}, \exampleName{Adder},
\exampleName{TwoBuyer}~\cite{HYC16},
\exampleName{OAuth}~\cite{RV13SPy},
\exampleName{TravelAgency}~\cite{ECOOP08SessionJava},
\exampleName{DistLogger}~\cite{ECOOP22AffineMPST}, and
\exampleName{CircBreaker}~\cite{ECOOP22AffineMPST}.
Notably,
\exampleName{DistLogger} and \exampleName{CircBreaker} are
inspired by real-world patterns in distributed computing.
\iftoggle{full}{We give details of the examples in \cref{sec:eval:examples}.}{}

We begin with the \emph{fully reliable} version of the examples,
and extend them to include crash handling behaviour.
Recall that our extended theory subsumes the original theory,
when all roles are assumed \emph{reliable}.
Therefore,
the fully reliable versions can act both as a sanity check,
to ensure the code generation does not exclude good protocols in the original
theory,
and as a baseline to compare against.

To add crash handling behaviour, we employ two patterns: \emph{failover} and
\emph{graceful failure}.
In a failover scenario,
a crashed role has its functions taken over by another role,
acting as a substitute to the crashed role~\cite{CONCUR22MPSTCrash}.
In a graceful failure scenario,
the protocol is terminated peacefully,
possibly involving additional messages for notification purposes.
Using the example from \cref{sec:overview},
the fully reliable protocol in \cref{ex:overview-global-without-crash}
is extended to one with graceful failure in
\cref{ex:overview-global-with-crash}.

We show a summary of the examples in \cref{tab:eval:table}.
For each example, we give the set of all roles $\roleSet$
and vary the set of reliable roles ($\rolesR$).
Each variant is given an identifier (Var.),
and each example always has a fully
reliable variant where $\rolesR = \roleSet$.
We give the number of communication interactions (Comms.),
the number of \gtCrashLab branches added (Crash Branches),
and the length of the longest continuation (Max Cont.\@ Len.)
in the given global type.


The largest of our examples in terms of concrete interactions is
\exampleName{OAuth}, with Variant $(i)$ having 26 interactions and $(j)$ having
30 interactions. This represents a $2.17\times$ and $2.5\times$ increase over
the size of the original protocol, and is a consequence of the confluence of two
factors: the graceful failure pattern, and low degree of branching in the
protocol itself. The \exampleName{TwoBuyer} Variant $(f)$ represents the
greatest increase ($2.57\times$) in interactions, a result of implementing the
failover pattern. The \exampleName{CircBreaker} variants are also notable in
that they are large in terms of both interactions and branching degree -- both
affect generation times.

\subparagraph*{Feasibility}\label{sec:eval:feasibility}

In order to demonstrate the feasibility of our tool \theTool, we give
generation times using our prototype for all protocol variants and examples,
plotted in \cref{fig:eval:stackedRuntimes}.
We show that \theTool is able to complete the code generation within
milliseconds,
which does not pose any major overhead for a developer.

\input{figs/resultsStackedBar.tex}

In addition to total generation times,
we report measurements for three main
constituent phases of \theTool: parsing, EffpiIR
generation, and code generation.
EffpiIR generation projects and transforms a parsed global type into an
intermediate representation,
which is then used to generate concrete \Scala code.

For all variants, the code generation phase is the most expensive
phase.
This is likely a consequence of traversing the given EffpiIR representation of
a protocol twice -- once for local type declarations and once for role-implementing
functions.
\iftoggle{full}{More details on generation time, including how they are measured, can be found in
\cref{sec:eval:times}.}{}


==> figs/implExample.tex <==
\begin{figure}
  {\small
  \begin{lstlisting}[language=effpi, gobble=4]
    // (i) label and payload declarations
    case class Log() // payload type
    case class Read() // label types
    case class Report(x : Log)
    case class Write(x : String) [*\hrule*]
    // (ii) recursion variable declarations
    sealed abstract class RecT0[A]() extends RecVar[A]("RecT0")
    case object RecT0 extends RecT0[Unit] [*\hrule*]
    // (iii) local type declarations
    type U[C0 <: OutChan[Read | Write], C1 <: InChan[Report]] = [*\label{line:effpi:U}*]
      Rec[RecT0,
          ( (Out[C0, Read] >>: In[C1, Report, (x0 : Report) => Loop[RecT0]]) [*\label{line:effpi:out_c0}*]
          | (Out[C0, Write] >>: Loop[RecT0]) )]

    type L[C0 <: InChan[Read | Write], C1 <: OutChan[Report]] = [*\label{line:effpi:L}*]
      Rec[RecT0,
          InErr[C0, Read | Write, (x0 : Read | Write) => L0[x0.type, C1], [*\label{line:effpi:recv-union}*]
                                  (err : Throwable) => PNil]]

    type L0[X0 <: Read | Write, C1 <: OutChan[Report]] <: Process =
      X0 match { case Read => Out[C1, Report] >>: Loop[RecT0] [*\label{line:effpi:recv-match}*]
                 case Write => Loop[RecT0] } [*\hrule*]
    // (iv) role-implementing functions
    def u(c0 : OutChan[Read | Write],
          c1 : InChan[Report]) : U[c0.type, c1.type] = {
      rec(RecT0) {
        val x0 = 0
        if (x0 == 0) {
          send(c0, new Read()) >> receive(c1) {(x1 : Report) => loop(RecT0) }
        } else {
          send(c0, new Write("")) >> loop(RecT0)
      } } }

    def l(c0 : InChan[Read | Write],
          c1 : OutChan[Report]) : L[c0.type, c1.type] =
      rec(RecT0) {
        receiveErr(c0)((x0 : Read | Write) => l0(x0, c1),
                       (err : Throwable) => nil) }

    def l0(x : Read | Write, c1 : OutChan[Report]) : L0[x.type, c1.type] =
      x match { case y : Read => send(c1, new Report(new Log())) >> loop(RecT0)
                case y : Write => loop(RecT0) } [*\hrule*]
    // (v) an entry point (main object)
    object Main {
      def main() : Unit = {
        var c0 = Channel[Read | Write]() [*\label{line:effpi:channel-create}*]
        var c1 = Channel[Report]()
        eval(par(u(c0, c1), l(c0, c1))) [*\label{line:effpi:channel-use}*]
    } }
  \end{lstlisting}
  }
  \caption{Generated \Scala code for the Simple Logger protocol in \Cref{fig:impl:egProtocol}}
  \label{fig:impl:egEffpi}
\end{figure}


==> figs/resultsMetrics.tex <==
\begin{table}[t]
  \caption{%
    Overview of All Variants for Each Example.
  }
  \vspace{-1em}
  \begin{center}
  \small
  \begin{tabular}{lCCccccc}
    \toprule
    Name & \text{Var.} & \rolesR & Comms.\@ & Crash Branches & Max Cont.\@
    Len.
    \\
    \midrule
    \multirow{2}{*}{%
      \begin{tabular}{@{}l@{}}
      \exampleName{PingPong} \\
      $\roleSet = \roleSetOf{p,q}$
      \end{tabular}
    } & (a) & \roleSet &	2 &	0 &	4 \\
     & (b) & \rolesEmpty &	2 &	2 &	4 \\\midrule
    \multirow{2}{*}{%
      \begin{tabular}{@{}l@{}}
      \exampleName{Adder} \\
      $\roleSet = \roleSetOf{p,q}$
      \end{tabular}
    } & (c) & \roleSet &	5 &	0 &	6 \\
     & (d) & \rolesEmpty &	5 & 5 &	6 \\\midrule
    \multirow{2}{*}{%
      \begin{tabular}{@{}l@{}}
      \exampleName{TwoBuyer} \\
      $\roleSet = \roleSetOf{p,q,r}$
      \end{tabular}
    } & (e) & \roleSet &	7 &	0 &	8 \\
     & (f) & \roleFmt{\{\roleR\}} &	18 & 6 &	12 \\\midrule
    \multirow{4}{*}{%
      \begin{tabular}{@{}l@{}}
      \exampleName{OAuth}\\
      $\roleSet = \roleSetOf{c,a,s}$
      \end{tabular}
    } & (g) & \roleSet &	12 &  0 &	11 \\
     & (h) & \roleFmt{\{s,a\}} &	21 & 8 &	11 \\
     & (i) & \roleFmt{\{s\}} &	26 & 13 &	11 \\
     & (j) & \rolesEmpty &	30 &	28 &	11 \\\midrule
    \multirow{3}{*}{%
      \begin{tabular}{@{}l@{}}
      \exampleName{TravelAgency}\\
      $\roleSet = \roleSetOf{c,a,s}$
      \end{tabular}
    } & (k) & \roleSet &	8 &	0 &	6 \\
     & (l) & \roleFmt{\{a,s\}} &	9 &	3 &	6 \\
     & (m) & \roleFmt{\{a\}} &	9 &	4 &	6 \\\midrule
    \multirow{3}{*}{%
      \begin{tabular}{@{}l@{}}
      \exampleName{DistLogger} \\
      $\roleSet = \roleSetOf{l,c,i}$
      \end{tabular}
    } & (n) & \roleSet &	10 &	0 &	7 \\
     & (o) & \roleFmt{\{i,c\}} &	15 &	2 &	7 \\
     & (p) & \roleFmt{\{i\}} &	16 &	4 &	7 \\\midrule
    \multirow{3}{*}{%
      \begin{tabular}{@{}l@{}}
      \exampleName{CircBreaker}\\
      $\roleSet = \roleSetOf{s,a,r}$
      \end{tabular}
    } & (q) & \roleSet &	18 &	0 &	10 \\
     & (r) & \roleFmt{\{a,s\}} &	24 &	3 &	10 \\
     & (s) & \roleFmt{\{a,s\}} &	23 &	3 &	11 \\
    \bottomrule
  \end{tabular}
  \end{center}
  \vspace{-1em}
  \label{tab:eval:table}
\end{table}


==> figs/resultsStackedBar.tex <==
\begin{figure}[t]
  \begin{center}
  \begin{tikzpicture}
    \begin{axis}[
        width=0.8\textwidth,
        height=3cm,
        enlargelimits=0.05,
        ybar stacked,
        bar width=0.7,
        ymajorgrids,
        scale only axis,
        xticklabels={$(a)$,$(b)$,$(c)$,$(d)$,$(e)$,$(k)$,$(l)$,$(m)$,$(n)$,$(g)$,$(o)$,$(p)$,$(f)$,$(q)$,$(h)$,$(s)$,$(r)$,$(i)$,$(j)$},
        xtick=data,
        ytick={0,0.5,...,2},
        xticklabel style={text height=2ex},
        minor y tick num=1,
        ylabel={Time (ms)},
        legend style={
          at={(0.3,0.95)},
          anchor=north,
          legend columns=-1,
          /tikz/every even column/.append style={column sep=1mm},
        },
      ]
      \pgfplotstableread{results/milliseconds.txt}\loadedtable
      \addplot table[x=Order, y=ReadFile] {\loadedtable};
      \addplot table[x=Order, y=EffpiGen] {\loadedtable};
      \addplot table[x=Order, y=ScalaGen] {\loadedtable};
      \legend{Parsing,EffpiIR,CodeGen};
    \end{axis}
  \end{tikzpicture}
  \end{center}
  \vspace{-2em}
  \caption{Average Generation Times for All Variants in
  \Cref{tab:eval:table}.}
  \vspace{-1em}
  \label{fig:eval:stackedRuntimes}
\end{figure}


==> implementation.tex <==
\section{\theTool: Generating Scala Programs from Protocols}
\label{sec:impl}

In this section, we present our toolchain \theTool for implementing our
extended MPST theory with crash-stop failures.
\theTool processes protocols represented in the \Scribble protocol
description language,
and generates protocol-conforming Scala code
that uses the \Effpi concurrency library.
A user specifies a multiparty protocol in \Scribble
as input, which we introduce in \cref{sec:impl:prelims}.
We show the style of our generated code in \cref{sec:impl:overview}, and how a
developer can use the generated code to implement multiparty protocols.
As mentioned in \cref{sec:overview},
generating channels for each process and type poses an interesting challenge,
and we explain it in \cref{sec:impl:boringdetail}.

\subsection{Specifying a Multiparty Protocol in \Scribble}
\label{sec:impl:prelims}

The \Scribble Language~\cite{YHNN2013} is a multiparty protocol
description language that relates closely to MPST theory
(\cf \cite{FeatherweightScribble}),
and provides a programmatic way to express global types.
As an example, \cref{fig:impl:egProtocol} describes the following global type
of a simple distributed logging protocol:

\smallskip
  {\centerline{
  \( {\small{
    \gtG =
    \gtRec{\gtFmt{\mathbf{t_{0}}}}{
      \gtCommRaw{\roleFmt{u}}{\roleFmt{l}}{
        \begin{array}{@{}l@{}}
          \gtCommChoice{\gtMsgFmt{write}}{\tyString}{ \gtFmt{\mathbf{t_{0}}} }
          \gtFmt{,}\quad
          \gtCommChoice{\gtMsgFmt{read}}{}{
            \gtCommSingle{\roleFmt{l}}{\roleFmt{u}}{\gtMsgFmt{report}}
                         {\stFmtC{Log}}{ \gtFmt{\mathbf{t_{0}}} }
          }
          \gtFmt{,}\quad
          \gtCommChoice{\gtCrashLab}{}{ \gtEnd }
        \end{array}
      }
    }
    }}
    .
  \)
  }}

\begin{figure}[t]
  \vspace{-1em}
  \begin{lstlisting}[language=Scribble,gobble=4]
    global protocol SimpleLogger(role U, reliable role L) [*\label{line:scribble:reliable}*]
    { rec t0 { choice at U { write(String) from U to L; [*\label{line:scribble:choice}*]
                             continue t0;               }
                        or { read from U to L;
                             report(Log) from L to U;
                             continue t0;               }
                        or { crash from U to L;         } } } [*\label{line:scribble:crash}*]
  \end{lstlisting}
  \vspace{-1.5em}
  \caption{A Simple Logger protocol in \Scribble.}
  \vspace{-.5em}
  \label{fig:impl:egProtocol}
\end{figure}


\smallskip
The global type is described by a \Scribble
\lstinline[language=Scribble]+global protocol+, with roles declared on
\cref{line:scribble:reliable}.
A transmission in the global type
(\eg $\gtCommRaw{\roleFmt{u}}{\roleFmt{l}}{\cdots}$)
is in the form of an interaction statement
(\eg \lstinline[language=Scribble]+... from U to L;+),
except that choice
(\ie with an index set $|I| > 1$) must be marked explicitly by a
\lstinline[language=Scribble]+choice+ construct (\cref{line:scribble:choice}).
Recursions and type variables in the global types are in the forms of
\lstinline[language=Scribble]+rec+ and \lstinline[language=Scribble]+continue+
statements, respectively.

In order to express our new theory,
we need two extensions to the language:
\begin{enumerate*}[label=\emph{(\arabic*)}]
  \item a reserved label \lstinline[language=Scribble]+crash+ to mark
    crash handling branches (\cf the special label $\gtCrashLab$ in the
    theory), \eg on \cref{line:scribble:crash}; and
  \item a \lstinline[language=Scribble]+reliable+ keyword to mark the reliable
    roles in the protocol (\cf the reliable role set $\rolesR$ in the theory).
    Roles are assumed unreliable unless declared using the
    \lstinline[language=Scribble]+reliable+ keyword, \eg \texttt{L} on
    \cref{line:scribble:reliable}.
\end{enumerate*}


\subsection{Generating \Scala Code from \Scribble Protocols}
\label{sec:impl:overview}

\subparagraph*{The \Effpi Concurrency Library}\!\!\!\!\cite{PLDI19Effpi}
provides an embedded Domain Specific Language (DSL) offering a simple
actor-based API\@.
The library utilises advanced type system features in Scala~3,
and provides both type-level and value-level constructs for processes and
channels.
In particular,
the type-level constructs reflect the behaviour of programs
(\ie processes), and thus can be used as specifications.
Following this intuition,
we generate process types that reflect local types from our theory,
as well as a tentative process implementing that type (by providing some
default values where necessary).



\input{figs/implExample.tex}

\subparagraph*{Generated Code}
To illustrate our approach,
we continue with the Simple Logger example from
\cref{sec:impl:prelims},
and show the generated code in \cref{fig:impl:egEffpi}.
The generated code can be divided into five sections:
\begin{enumerate*}[label=\emph{(\roman*)}]
\item label and payload declarations,
\item recursion variable declarations,
\item local type declarations,
\item role-implementing functions, and
\item an entry point.
\end{enumerate*}

Sections \emph{(i)} and \emph{(ii)} contain boilerplate code,
where we generate type declarations for various constructs needed for
expressing local types and processes.
We draw attention to the \emph{key} sections \emph{(iii)} and \emph{(iv)},
where we generate a representation of local types for each role,
as well as a tentative process inhabiting that type.

\subparagraph*{Local Types and \Effpi Types}
We postpone the discussion about channels in \Effpi to
\cref{sec:impl:boringdetail}.
For now, we
compare the generated \Effpi type and the projected local type,
and also give a quick primer\footnotemark\ on \Effpi constructs.
The projected local types of the roles $\roleFmt{u}$ and $\roleFmt{l}$ are
shown as follows:

\footnotetext{A more detailed description of constructs can be found
in~\cite{SCALA19Effpi}.}

\smallskip
\centerline{
\(
{\small{
\begin{array}{rcl}
\gtProj[\setenum{\roleFmt{l}}]{\gtG}{\roleFmt{u}}
& = &
\stRec{\stFmt{\mathbf{t_{0}}}}{
  \stIntSum{\roleFmt{l}}{}{
    \begin{array}{@{}l@{}}
      \stChoice{\stMsgFmt{write}}{\tyString} \stSeq \stFmt{\mathbf{t_{0}}}
      \stFmt{,}\quad
      \stChoice{\stMsgFmt{read}}{}
      \stSeq
      \stInNB{\roleFmt{l}}{\stMsgFmt{report}}{\stFmtC{Log}}{
        \stFmt{\mathbf{t_{0}}}
      }

    \end{array}
  }
} \\
\gtProj[\setenum{\roleFmt{l}}]{\gtG}{\roleFmt{l}}
& = &
\stRec{\stFmt{\mathbf{t_{0}}}}{
  \stExtSum{\roleFmt{u}}{}{
    \begin{array}{@{}l@{}}
      \stChoice{\stMsgFmt{write}}{\tyString} \stSeq \stFmt{\mathbf{t_{0}}}
      \stFmt{,}\quad
      \stChoice{\stMsgFmt{read}}{}
      \stSeq
      \stOut{\roleFmt{u}}{\stMsgFmt{report}}{\stFmtC{Log}}
      \stSeq
      \stFmt{\mathbf{t_{0}}}
      \stFmt{,}\quad
      \stChoice{\stCrashLab}{} \stSeq {\stEnd}
    \end{array}
  }
}
\end{array}
}
}
\)
} %

\smallskip
\noindent
The local types are recursive,
and the \Effpi type implements recursion with
\lstinline[language=Effpi]+Rec[RecT0, ...]+
and
\lstinline[language=Effpi]+Loop[RecT0]+,
using the recursion variable \texttt{RecT0} declared in section \emph{(ii)}.

For role \roleFmt{u},
The inner local type is a sending type towards role $\roleFmt{l}$,
and we use an \Effpi process output type
\lstinline[language=Effpi]+Out[A, B]+,
which describes a process that uses a channel of type \texttt{A} to send a value
of type \texttt{B}.
For each branch, we use a separate output type, and connect it to
the type of the continuation using a
sequential composition operator (\lstinline[language=Effpi]+>>:+).
The different branches are then composed together
using a union type (\texttt{|}) from the \Scala~3 type system.

Recall that the role $\roleFmt{l}$ is declared
\lstinline[language=Scribble]+reliable+,
and thus the reception labelled \texttt{report} from \roleFmt{l} at \roleFmt{u}
does not need to contain a crash handler.
We use an \Effpi process input type
\lstinline[language=Effpi]+In[A, B, C]+,
which describes a process that uses a channel of type \texttt{A} to receive a
value of type \texttt{B}, and uses the received value in a continuation of type
\texttt{C}.

For role \roleFmt{l}, the reception type is more complex for two reasons:
\begin{enumerate*}[label=\emph{(\arabic*)}]
  \item role $\roleFmt{u}$ is unreliable, necessitating crash handling; and
  \item the reception contains branching behaviour (\cf the reception
    \roleFmt{u} is a singleton case), with labels \texttt{write} and
    \texttt{read}.
\end{enumerate*}
To address the former, we extend \Effpi with a variant of the input process type
\lstinline[language=Effpi]+InErr[A, B, C, D]+,
where \texttt{D} is the type of continuation in case of a crash.
To address the latter, the payload type is first received as an union
(\cref{line:effpi:recv-union}), and then pattern matched to select the
correct continuation according to the type (\cref{line:effpi:recv-match}).

\subparagraph*{From Types To Implementations}
Since \Effpi type-level and value-level constructs are closely related,
we can easily generate the processes from the processes types.
Namely, by matching
the type \lstinline[language=effpi]+Out[..., ...]+
with the process \lstinline[language=effpi]+send(..., ...)+;
the type \lstinline[language=effpi]+In[..., ...]+
with the process \lstinline[language=effpi]+receive(...) {... => ...}+;
and similarly for other constructs.
Whilst executable, the generated code represents a skeleton implementation,
and the programmer is expected to alter the code according to their
requirements.

We also introduce a new crash handling receive process
\lstinline[language=effpi]+receiveErr+,
to match the new \lstinline[language=Effpi]+InErr+ type.
Process crashes are modelled by (caught) exceptions and errors in
role-implementing functions, %
and crash detection is achieved via timeouts.
Timeouts are set by the programmer in an
(implicit) argument to each \lstinline[language=effpi]+receiveErr+ call.

Finally,
the entry point (main object) in section \emph{(v)}
composes the role-implementing functions together with
\lstinline[language=effpi]+par+ construct in \Effpi,
as well as connecting the processes together with channels.








\subsection{Generating \Effpi Channels from Scribble Protocols}
\label{sec:impl:boringdetail}

As previously mentioned,
\Effpi processes use \emph{channels} to communicate,
and the type of the channel is reflected in the type of the process.
However, our local types do not have any channels;
instead, they contain a partner role with which to communicate.
This poses an interesting challenge,
and we explain the channel generation procedure in this section.

We draw attention to the generated code in \cref{fig:impl:egEffpi} again,
where we now focus on the parameters \texttt{C0} in the generated types
\texttt{U} and \texttt{L}.
In the type \texttt{U}, the channel type \texttt{C0} needs to be a subtype of
\lstinline[language=effpi]+OutChan[Read | Write]+ (\cref{line:effpi:U}),
and we see the channel is used in the output processes types, \eg
\lstinline[language=effpi]+Out[C0, Read]+
(\cref{line:effpi:out_c0},
note that output channels subtyping is covariant on the payload type).
Dually, in the type \texttt{L}, the channel type \texttt{C0} needs to be a
subtype of
\lstinline[language=effpi]+InChan[Read | Write]+ (\cref{line:effpi:L}),
and we see the channel is used in the input process type, \ie
\lstinline[language=effpi]+InErr[C0, Read | Write, ..., ...]+
(\cref{line:effpi:recv-union}).

Similarly,
a channel \texttt{c0} is needed in the role-implementing functions
\texttt{u} and \texttt{l} as arguments,
and the channel is used in processes
\lstinline[language=effpi]+send(c0, ...)+ and
\lstinline[language=effpi]+receiveErr(c0) ...+.
Finally, in the entry point, we create a bidirectional channel
\lstinline[language=effpi]+c0 = Channel[Read | Write]()+
(\cref{line:effpi:channel-create}),
and pass it as an argument to the role-implementing functions \texttt{u} and \texttt{l}
(\cref{line:effpi:channel-use}),
so that the channel can be used to link two role-implementing processes
together for communication.

Generating the channels correctly is crucial to the correctness of our
approach,
but non-trivial in the meantime since channels are implicit in the protocols.
In order to do so, a simple approach is to
traverse each interaction in the global protocol,
and assign a channel to each accordingly.

This simple approach would work for the example we show in
\cref{fig:impl:egProtocol};
however, it would not yield the correct result when \emph{merging} occurs
during projection, which we explain using an example.
For clarity and convenience, we use \emph{annotated} global and local types,
where we assign an identifier for each interaction to signify the channel to
use,
and consider the following global type:

\smallskip
\centerline{
\(
  \gtG = \gtCommRawAnn{\roleP}{\roleQ}{0}{
    \gtCommChoice{\gtLabFmt{left}}{}{
      \gtCommSingleAnn{\roleP}{\roleR}{1}{\gtLabFmt{left}}{}{\gtEnd}
    }
    \gtFmt{,} \quad
    \gtCommChoice{\gtLabFmt{right}}{}{
      \gtCommSingleAnn{\roleP}{\roleR}{2}{\gtLabFmt{right}}{}{\gtEnd}
    }
  }
\)
}%

\smallskip
The global type describes a simple protocol, where role $\roleP$ selects a
label \gtLabFmt{left} or \gtLabFmt{right} to $\roleQ$, and $\roleQ$ passes on
the same label to $\roleR$.
As a result, the projection on $\roleR$ (assuming all roles reliable) should
be a reception from $\roleQ$ with branches labelled $\gtLabFmt{left}$ or
$\gtLabFmt{right}$, \ie
\(
  \stExtSumAnn{\roleP}{1,2}{}{
      \stChoice{\stLabFmt{left}}{} \stSeq \stEnd
      \stFmt{,}\quad
      \stChoice{\stLabFmt{right}}{} \stSeq \stEnd
  }
\).
Here, we notice that the interaction between $\roleQ$ and $\roleR$ should take
place on a single channel, instead of two separate channels annotated $1$ and
$2$.

When \emph{merging} behaviour occurs during projection,
we need to use the same channel in those interactions
to achieve the correct behaviour.
After traversing the global type to annotate each interaction,
we use a union-find data structure to merge annotations involved in merges
during projection. \iftoggle{full}{Additional technical details are included in \cref{sec:appendix:channel-gen}.}{}

